Stochastic Bandits with Delay-Dependent Payoffs

Motivated by recommendation problems in music streaming platforms, we propose a nonstationary stochastic bandit model in which the expected reward of an arm depends on the number of rounds that have passed since the arm was last pulled. After proving that finding an optimal policy is NP-hard even when all model parameters are known, we introduce a class of ranking policies provably approximating, to within a constant factor, the expected reward of the optimal policy. We show an algorithm whose regret with respect to the best ranking policy is bounded by $\widetilde{\mathcal{O}}\big(\!\sqrt{kT}\big)$, where $k$ is the number of arms and $T$ is time. Our algorithm uses only $\mathcal{O}\big(k\ln\ln T\big)$ switches, which helps when switching between policies is costly. As constructing the class of learning policies requires ordering the arms according to their expectations, we also bound the number of pulls required to do so. Finally, we run experiments to compare our algorithm against UCB on different problem instances.

==> old_experiments.tex <==
\section{Experiments} \label{Sec:Experiments}
In this section we present an empirical evaluation of the \low policy run in a synthetic environment.
\paragraph{Setup.} We create an ad hoc environment with the aim of analyzing the learning as a function of the different setting parameters without introducing too much variance. Variance that we would have suffered if we had generated all the parameters fully randomly. We first present the adopted baseline reward expectation assignment approach. We start by assigning arm means as $b$ evenly spaced numbers over the $[0,1]$ interval. Clearly, the more the values, the closer is the gap between consecutive baseline expectations $\Delta_{i,i+1}$. Then we create another set of baseline expectations as evenly spaced number over the smaller interval $[1,f]$, where $f$ stands for \textit{fraction of top-arms} and is our first running parameter. The final set of arm means is given by the union of these sets of values, which will be dense over the interval $[1,f]$ and more scattered over the rest of the interval $[f,0]$. The unknown arm-dependent parameters $d_i$ were generated as random integers in the set $\{1,\dots,D\}$, where the max-delay $D$ is our second running parameter. Finally, we consider rewards as random variates of a Bernoulli distribution whose parameter is defined according to Equation \ref{Eq:Payout}, where we set $f(\tau) = \gamma^\tau$ and the discount factor $\gamma \in (0,1)$ is our last running parameter.

\paragraph{Benchmarks.} Given the hardness result stated in Theorem \ref{Th:Hardness}, in the empirical analysis we compare against the \textit{ghost} policy defined in Section \ref{Sec:RegretDec}. Our main competitor is named \piucb and consists of running UCB1 on top of the Bandit Ranker procedure instead of the action elimination approach adopted in \low. Finally, in order to observe the influence of the non-stationary effect in the payoff functions, we compare also against the standard UCB1 policy.

\paragraph{Results.} The experiments we present in this section measure cumulative reward throughout time. The arms have been generated by setting $b=6$ and considering different values of $f$ and they were all run over $T=1000000$ rounds. It is natural to notice that according to the value of the non-stationary parameters $\gamma$ and $\overline{d}$, the non-stationary effect may bring a different influence in the expected reward. As we want to restric our attention to the different behaviours observed with respect to the strength of the non-stationarity, the provided results are therefore aligned by different values of $\gamma$ and $\overline{d}$. In particular, we split them in three cases according to the different values of $\gamma$, which controls the discount effect.
\begin{figure*}
  \centering
  \includegraphics[width=5cm]{{g0.2_ft0.1_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.5_ft0.1_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.999_ft0.1_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}\\
%
  \includegraphics[width=5cm]{{g0.2_ft0.1_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.5_ft0.1_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.999_ft0.1_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}\\
 %
  \includegraphics[width=5cm]{{g0.2_ft0.3_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.5_ft0.3_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.999_ft0.3_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}\\
%
  \includegraphics[width=5cm]{{g0.2_ft0.3_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.5_ft0.3_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.999_ft0.3_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}\\
%
  \includegraphics[width=5cm]{{g0.2_ft0.5_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.5_ft0.5_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.999_ft0.5_d0.1_dUB5_dBar7_bin1_T200000_k6}.png}\\
%
  \includegraphics[width=5cm]{{g0.2_ft0.5_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.5_ft0.5_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}
  \includegraphics[width=5cm]{{g0.999_ft0.5_d0.1_dUB5_dBar9_bin1_T200000_k6}.png}\\
%
  \caption{Comparison of \textit{greedy}, \textit{ghost}, \textit{UCB1} with our solution \textit{FPO}. The results were obtained with different configurations of the non-stationary parameters. Note that, the gap between our solution and the baselines is strongly affected by the value of $\gamma$.
}
\label{fig:cumulative_reward}
\end{figure*}

==> open_problems.tex <==
\begin{enumerate}
    \item doubling trick to reduce number of pulls.
    \item search for a better approximation when we are not in the case that \ghost is optimal.
\end{enumerate}

==> preamble.tex <==
\twocolumn[

\aistatstitle{Latent Combination with Non-stationary Combinatorial Bandits}

\aistatsauthor{ Leonardo Cella \And Nicol\`{o} Cesa-Bianchi }
\vspace{2mm}
\aistatsaddress{Dipartimento di Informatica, University of Milan, Italy } ]

